Spectral Characterization and Mitigation of Sequential Knowledge Editing Collapse

Sequential knowledge editing in large language models often causes catastrophic collapse of the model's general abilities, especially for parameter-modifying methods. Existing approaches mitigate this issue through heuristic constraints on parameter updates, yet the mechanisms underlying such degradation remain insufficiently understood. In this work, we present a spectral analysis of sequential knowledge editing and show that a model's general abilities are closely associated with dominant singular directions of pretrained weight matrices. These directions are highly sensitive to perturbations and are progressively disrupted by repeated edits, closely tracking the collapse in both editing efficacy and general performance. Building on this insight, we propose REVIVE, a plug-and-play framework that stabilizes sequential editing by explicitly preserving the dominant singular subspace. REVIVE represents parameter updates in the spectral basis of the original weights and filters components that would interfere with the protected region. Extensive experiments across multiple models and benchmarks show that REVIVE consistently improves editing efficacy while substantially preserving general abilities under long-horizon sequential editing, including extreme settings with up to 20,000 edits.

==> name.tex <==
\section{Comparison with Other SVD-based Editing Methods}
\label{app:svd_comparison}

In this section, we provide a focused comparison between \textbf{REVIVE} and representative prior editing methods that also employ SVD or subspace constraints, including \textbf{AlphaEdit}, \textbf{PRUNE}, and \textbf{Delta-Edit}.
Although these methods share a superficial similarity in that they all regulate updates via low-rank or projection-based mechanisms, they differ fundamentally in \emph{(i)} the source of the protected subspace, \emph{(ii)} the failure mode they are designed to address, and \emph{(iii)} the scope of degradation they can prevent.

\paragraph{AlphaEdit.}
AlphaEdit constructs a protected subspace from the covariance of feature activations induced by a large external factual dataset (e.g., 100k triples).
Its goal is to reduce interference between factual representations during sequential edits.
As a result, the protected subspace is \emph{extrinsic} and tightly coupled to the sampled data distribution.
While this strategy is effective in early editing stages, it does not prevent the gradual corruption of the model’s intrinsic operator structure.
Empirically, AlphaEdit exhibits severe degradation after long edit sequences, with both editing efficacy and general abilities collapsing after approximately 8k edits.

\paragraph{PRUNE.}
PRUNE regulates updates by constraining the singular values of the update matrix, preventing them from exceeding the maximum singular value of the original weights.
This mechanism focuses solely on update magnitude and does not distinguish between different singular directions.
Consequently, PRUNE may suppress useful update components while failing to preserve the functional subspace that supports general model abilities.
It is therefore not designed to address long-horizon degradation caused by directional drift in the parameter spectrum.

\paragraph{Delta-Edit.}
Delta-Edit (and related O-Edit methods) explicitly targets \emph{edit--edit interference}.
By tracking past gradient or update directions and projecting new edits to be orthogonal to them, these methods aim to prevent overwriting previous edits.
However, their protected subspace is derived entirely from \emph{historical edit directions}, rather than from the intrinsic structure of the pretrained model.
As a result, Delta-Edit does not address model-level spectral drift and cannot prevent the gradual degradation of general abilities that occurs even when edits are semantically unrelated.

\paragraph{REVIVE (ours).}
REVIVE is motivated by a different and previously unaddressed failure mode: the progressive corruption of the \emph{dominant singular subspace} of FFN weight matrices during long edit sequences.
Through spectral analysis, we identify that high-energy singular directions encode the model’s general abilities.
REVIVE therefore protects an \emph{intrinsic}, model-derived subspace defined by the dominant singular vectors of the weights themselves.
By selectively filtering update components that distort this subspace, REVIVE prevents spectral degradation and enables stable editing beyond 20k sequential edits.

\begin{table*}[t]
\centering
\caption{Comparison between REVIVE and representative SVD-based or subspace-constrained editing methods.}
\label{tab:svd_comparison}
\renewcommand{\arraystretch}{1.05}
\resizebox{\textwidth}{!}{%
\begin{tabular}{p{2.8cm} p{4.6cm} p{4.2cm} p{5.0cm} p{5.6cm}}
\toprule
\textbf{Method} &
\textbf{Protected Subspace Source} &
\textbf{Target Failure Mode} &
\textbf{Limitation} &
\textbf{Difference vs.\ REVIVE} \\
\midrule
\textbf{AlphaEdit} &
Feature covariance from \textbf{external factual data} (e.g., 100k triples) &
Interference across factual activations &
Subspace is \textbf{extrinsic} and data-dependent; performance collapses after long edit sequences &
REVIVE protects an \textbf{intrinsic spectral structure} derived directly from model weights \\
\textbf{PRUNE} &
Singular values constrained by original $\sigma_{\max}$ &
Overly large parameter updates &
Magnitude-only filtering ignores singular \textbf{directions} and functional roles &
REVIVE selectively filters \textbf{harmful directions} while preserving general abilities \\
\textbf{Delta-Edit} &
Accumulated \textbf{past edit / gradient directions} &
Edit--edit interference &
Only resolves conflicts between edits; does not prevent intrinsic model drift &
REVIVE targets \textbf{spectral degradation} independent of edit history \\
\textbf{REVIVE (ours)} &
Dominant singular vectors of FFN weight matrices &
Collapse due to \textbf{dominant subspace corruption} &
-- &
Enables \textbf{20k+ stable edits} by addressing a previously unidentified failure mode \\
\bottomrule
\end{tabular}
}
\end{table*}

\paragraph{Summary.}
Although prior methods employ projection or low-rank constraints, they differ fundamentally from REVIVE in both motivation and mechanism.
AlphaEdit and Delta-Edit focus on \emph{interference control} (across data or across edits), while PRUNE enforces coarse magnitude constraints.
REVIVE is the first method to identify and directly mitigate \emph{spectral degradation of the dominant singular subspace} as the root cause of long-horizon sequential editing failure, providing a principled and scalable solution for sustained knowledge editing.

